Revisiting Optimal Resilience of Fast Byzantine Consensus (Extended Version)

It is a common belief that Byzantine fault-tolerant solutions for consensus are significantly slower than their crash fault-tolerant counterparts. Indeed, in PBFT, the most widely known Byzantine fault-tolerant consensus protocol, it takes three message delays to decide a value, in contrast with just two in Paxos. This motivates the search for fast Byzantine consensus algorithms that can produce decisions after just two message delays \emph{in the common case}, e.g., under the assumption that the current leader is correct and not suspected by correct processes. The (optimal) two-step latency comes with the cost of lower resilience: fast Byzantine consensus requires more processes to tolerate the same number of faults. In particular, $5f+1$ processes were claimed to be necessary to tolerate $f$ Byzantine failures. In this paper, we present a fast Byzantine consensus algorithm that relies on just $5f-1$ processes. Moreover, we show that $5f-1$ is the tight lower bound, correcting a mistake in the earlier work. While the difference of just $2$ processes may appear insignificant for large values of $f$, it can be crucial for systems of a smaller scale. In particular, for $f=1$, our algorithm requires only $4$ processes, which is optimal for any (not necessarily fast) partially synchronous Byzantine consensus algorithm.

==> drafts/exec_3.tex <==
\paragraph{Execution $\exec_3$.}
First, let us look at what happened during the second round \atadd{in executions $\exec_2$ and $\exec_4$}.
We define two relations $S$ and $R$ on $X = \{p, P_1, P_2, P_3, P_4, P_5\}$.
% where $(x, y) \in S$ (resp. $R$) means that in both $\exec_2$ and $\exec_4$, $x$ sent $y$ the same messages (resp. $y$ received the same messages from $x$) during the \atreplace{round $[\Delta, 2\Delta)$}{second round}.
$(x,y) \in S$ means that in both $\exec_2$ and $\exec_4$, $x$ sent to $y$ the same messages at the same time and in the same order during the second round (i.e., time interval $[\Delta, 2\Delta)$).
$(x, y) \in R$ means that in both $\exec_2$ and $\exec_4$, $x$ received from $y$ the same set of messages at the same time and in the same order during the third round (i.e., time interval $[2\Delta, 3\Delta)$).

In the second round of executions $\exec_2$ and $\exec_4$:
\begin{itemize}
    % \item $p$ \yzreplace{is Byzantine so it is possible for us to assume that $p$ sends the same messages to each $P_i$ during the two executions.}{was silent to $P_1$, $P_2$, $P_4$, $P_5$ in both executions, so $(p, y) \in R \cap S$ for all $y \in \{P_1, P_2, P_4, P_5\}$.}
    \item $p$ was silent to $P_1$, $P_2$, $P_4$, $P_5$ in both executions, so $(p, y) \in R \cap S$ for all $y \in \{P_1, P_2, P_4, P_5\}$.
    
    % \item \yzrev{$P_1$ and $P_5$ were correct and started with the same state after the first round in both $\exec_2$ and $\exec_4$. This means $(P_1, y), (P_5, y) \in S$ for all $y \in X$. Since their messages to everyone except $P_3$ were delivered on time, we also have have $(P_1, y)$, $(P_5, y) \in R$ for all $y \in X \setminus \{P_3\}$.}
    %
    \item Group $P_1$ was correct and received the same messages at the same time and in the same order in the second round in both $\exec_2$ and $\exec_4$.
    The same applies to group $P_5$.
    Since we only consider deterministic processes, $(P_1, y), (P_5, y) \in S$ for all $y \in X$.
    Since their messages to everyone except $P_3$ were delivered on time, we also have have $(P_1, y)$, $(P_5, y) \in R$ for all $y \in X \setminus \{P_3\}$.
    
    % \item \yzreplace{In $\exec_2$, the Byzantine $P_2$ sent the same message deliveries to everyone besides $P_3$ $P_1$, $P_4$, and $P_5$ as its correct version did in $\exec_4$; In $\exec_4$, the Byzantine $P_4$ sent the same message deliveries to $P_1$, $P_2$, and $P_5$ as its correct version did in $\exec_2$;}{Both $P_2$'s Byzantine version in $\exec_2$ and the correct version in $\exec_4$ \atreplace{emulated}{acted in the same way as in} $\exec_5$ when interacting with the non-$P_3$ groups and \atreplace{emulated}{in the same way as in} $\exec_1$ when interacting with $P_3$. A similar logic holds for $P_4$, so $(P_2, y)$, $(P_4, y) \in R \cap S$ for all $y \in X$. (TODO: careful about receiving times and definition of R. Also, it's important that you can't give $P_3$ enough time to respond during the round, since that may cause further interactions)}
    %
    \item Both $P_2$'s Byzantine version in $\exec_2$ and the correct version in $\exec_4$ acted in the same way as in $\exec_5$ when interacting with the non-$P_3$ groups.
    Similarly, $P_4$ acted as in $\exec_1$ in both $\exec_2$ and $\exec_4$ for all the non-$P_3$ groups.
    Hence, $(P_2, y)$, $(P_4, y) \in R \cap S$ for all $y \in X \setminus \{P_3\}$.
    
    % \item \yzadd{$P_3$ is correct but behaves differently in $\exec_2$ and $\exec_4$, so it sends different messages to other processes. However, since it was slow during the second rounds of both executions, we have $(P_3, y) \in R$ for all $y \in X$.}
    \item $P_3$ is correct but behaves differently in $\exec_2$ and $\exec_4$, so it sends different messages to other processes.
    However, since its messages are delayed, no process hears from $P_3$ in the third round.
    Hence, $(P_3, y) \in R$ for all $y \in X$.
\end{itemize}
% \yzremove{The important point is this: \textbf{after the second round, we can assume that every non-$P_3$ process has the same state (or if Byzantine in at least one execution, can act as if it were in the same state) in the two executions $\exec_2$ and $\exec_4$.}}
We can check that:
\begin{itemize}
    \item $\forall x \in X$ and $\forall y \in \{P_1, P_2, P_4, P_5\}$, $(x, y) \in R$;
    \item $\forall x \in \{P_1, P_2, P_4, P_5\}$ and $\forall y \in X$, $(x, y) \in S$;
\end{itemize}
%
Therefore, we can continue both $\exec_2$ and $\exec_4$
% \yzremove{(as long as $P_3$'s pending messages do not reach anyone)}
as if the processes in $P_1 \cup P_2 \cup P_4 \cup P_5$ were the only correct processes
% \yzreplace{starting from some state $r$ after completing their second step.}{...}
in some partial execution that just finished its second round, where the Byzantine processes $\{p\} \cup P_3$ all crashed permanently at the end of the first round (recall that in $\exec_2$ and $\exec_4$ $p$ sends no messages in the second round except to $P_3$). Since there are only $f$ processes in $\{p\} \cup P_3$,
% \yzremove{We now construct $\exec_3$. Recall that $\{p\} \cup P_3$ are Byzantine. We let all processes in $P_3$ crash permanently at the end of the first round. The key idea with $\exec_3$ is that by the discussion we just had, we can assume that after the second round its (correct) processes $P_1 \cup P_2 \cup P_4 \cup P_5$ are in the same group state $c$ as their counterparts in $\exec_2$ and $\exec_4$. Since there are only $f$ Byzantine processes total,}
by the {\liveness} property of consensus there must exist a continuation of our partial execution that obtains consensus at some moment $T$. We pick this execution to be $\exec_3$.


==> figures/equivocation-quorum-intersection.tex <==
\begin{figure}%{r}{0.4\textwidth}
\begin{subfigure}[t]{0.47\textwidth}
    \centering
    \customincludesvg{svg/equivocation-quorum-intersection-1.svg}
    \caption{Normal case execution example.
    $\tauHat = \fsign_p(\MPropose, \xHat, v)$, where $p$ is the identifier of the leader process that sends the {\MPropose} message.
    $\sigAck = \fsign_q(\MAck, \xHat, v)$, where $q$ is the identifier of the process that sends the {\MAck} message.}
    \label{subfig:normal-case-example}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.47\textwidth}
    \centering
    \customincludesvg{svg/view-change-example.svg}
    \caption{\needsrevA{View change execution example. $\vote = (x, u, \sigma, \tau)$. $\sigVote = \fsign_q(\MVote, \vote)$ and $\sigCertAck = \fsign_q(\MCertAck, \xHat, v)$, where $q$ is the identifier of the process that sends the {\MVote} and {\MCertAck} messages.}}
    \label{subfig:view-change-example}
\end{subfigure}

\caption{\addA{Execution examples of our protocol.}}
\label{fig:execution-examples}
\end{figure}


==> sections/discussion.tex <==
\section{Discussion}

State machine replication?
External validity?

Open questions: other optimistic assumptions, ?








